What should I document? A preliminary systematic mapping study into API documentation knowledge

Background: Good API documentation facilities the development process, improving productivity and quality. While the topic of API documentation quality has been of interest for the last two decades, there have been few studies to map the specific constructs needed to create a good document. In effect, we still need a structured taxonomy against which to capture knowledge. Aims: This study reports emerging results of a systematic mapping study. We capture key conclusions from previous studies that assess API documentation quality, and synthesise the results into a single framework. Method: By conducting a systematic review of 21 key works, we have developed a five dimensional taxonomy based on 34 categorised weighted recommendations. Results: All studies utilise field study techniques to arrive at their recommendations, with seven studies employing some form of interview and questionnaire, and four conducting documentation analysis. The taxonomy we synthesise reinforces that usage description details (code snippets, tutorials, and reference documents) are generally highly weighted as helpful in API documentation, in addition to design rationale and presentation. Conclusions: We propose extensions to this study aligned to developer's utility for each of the taxonomy's categories.

==> preamble/extended/authblk.tex <==
%\usepackage{authblk}
%\renewcommand*{\Authsep}{, }
%\renewcommand*{\Authand}{, }
%\renewcommand*{\Authands}{, }
%\renewcommand*{\Affilfont}{\normalsize\normalfont}

==> preamble/simple.tex <==
\usepackage{hyperref}
\input{simple/author}
\input{simple/captions}
\input{simple/cleverref}
\input{simple/geometry}
\input{simple/graphics}
\input{simple/typesetting}

==> preamble/simple/author.tex <==
\author{Alex Cummaudo\\Applied Artificial Intelligence Institute\\Deakin University, Australia}
\date{\today}


==> preamble/simple/captions.tex <==
\usepackage[labelfont=bf]{caption}

==> preamble/simple/cleverref.tex <==
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}
\Crefname{lstlisting}{Listing}{Listings}

==> preamble/simple/geometry.tex <==
\usepackage{geometry}
\newgeometry{top=2.25cm,right=2cm,bottom=2.5cm,left=3cm}


==> preamble/simple/graphics.tex <==
\usepackage{graphicx}
\graphicspath{{images/}{../images/}}


==> preamble/simple/typesetting.tex <==
% Linespread of 1.5 as required by SIT
\linespread{1.5}
% Times new roman package
\usepackage{mathptmx}
% Change font style for sub-sub section
\usepackage{sectsty}
\subsubsectionfont{\normalfont\itshape}
